DSeq-JEPA: Discriminative Sequential Joint-Embedding Predictive Architecture

Recent advances in self-supervised visual representation learning have demonstrated the effectiveness of predictive latent-space objectives for learning transferable features. In particular, Image-based Joint-Embedding Predictive Architecture (I-JEPA) learns representations by predicting latent embeddings of masked target regions from visible context. However, it predicts target regions in parallel and all at once, lacking ability to order predictions meaningfully. Inspired by human visual perception, which attends selectively and progressively from primary to secondary cues, we propose Dseq-JEPA, a Discriminative Sequential Joint-Embedding Predictive Architecture that bridges latent predictive and autoregressive self-supervised learning. Specifically, Dseq-JEPA integrates a discriminatively ordered sequential process with JEPA-style learning objective. This is achieved by (i) identifying primary discriminative regions using an attention-derived saliency map that serves as a proxy for visual importance, and (ii) predicting subsequent regions in discriminative order, inducing a curriculum-like semantic progression from primary to secondary cues in pre-training. Extensive experiments across tasks -- image classification (ImageNet), fine-grained visual categorization (iNaturalist21, CUB, Stanford Cars), detection/segmentation (MS-COCO, ADE20K), and low-level reasoning (CLEVR) -- show that Dseq-JEPA consistently learns more discriminative and generalizable representations compared to I-JEPA variants.

==> figures/patch_clustering.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
% \begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Patch_clustering-v2.pdf}
    \caption{\textbf{Evolution of patch-level clustering during pre-training.} From left to right: input image and 4-cluster results from ViT-B/16 checkpoints at 150, 300, 450, and 600 epochs.}
    \label{fig:patch_cluster}
% \end{figure}
\end{wrapfigure}

==> figures/per_step_prediction.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/per_step_prediction_f.pdf}
%     \caption{\textbf{Per-step prediction difficulty for DSeq-JEPA (ViT-B/16)}. We report the average prediction loss on 10{,}000 ImageNet images when predicting the Top-2, Top-3, Top-4, and Top-5 discriminative regions, using the checkpoint at epoch 450.}
%     \label{fig:per_step}
% \end{figure}

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    % \vspace{-1.7\baselineskip} % optional: tighten top spacing
    \includegraphics[width=0.5\textwidth]{figures/per_step_prediction_f.pdf}
    \setlength{\abovecaptionskip}{0.1cm}
    \caption{\textbf{Per-step prediction difficulty for DSeq-JEPA (ViT-B/16)}. We report the average prediction loss on 10{,}000 ImageNet images when predicting the Top-2, Top-3, Top-4, and Top-5 discriminative regions, using the checkpoint at epoch 450.}
    \label{fig:per_step}
    \vspace{-1.8\baselineskip} % optional: tighten bottom spacing
\end{wrapfigure}

==> table/cls_token.tex <==
% \begin{table}[t]
%   \caption{\textbf{Effects of class token.} }
%   \label{tab:clstoken}
%   \centering
%   \begin{tabular}{>{\centering\arraybackslash}m{4.8cm} >{\centering\arraybackslash}m{2.5cm}}
%     \toprule
%     \textbf{Method} & \textbf{ImageNet} \\
%     \midrule
%     \midrule
%     I-JEPA & 72.4\\
%     I-JEPA w/ \texttt{[CLS]} & 72.4 \\
%     % \textbf{\ours~w/o \texttt{[CLS]}} & \\ %66.1 \\
%     % \rowcolor{lightblue}
%     % \textbf{\ours} &  \textbf{73.5}\\
%     \bottomrule
%   \end{tabular}
% \end{table}
% \begin{table}[h]
%   \caption{\textbf{Effect of class token.} }
%   \label{tab:clstoken}
%   \centering
%   \begin{tabular}{ccc}
%     \toprule
%     \textbf{Method} & I-JEPA &  +\texttt{[CLS]}\\
%     \midrule
%     \midrule
%     \textbf{ImageNet} & 72.4 & 72.4 \\
%     \bottomrule
%   \end{tabular}
% \end{table}
\begin{table}[t]
\centering
\begin{minipage}[t]{0.4\linewidth}
  \centering
  \caption{\textbf{Effect of class token.} }
  \label{tab:clstoken}
    \begin{tabular}{ccc}
    \toprule
    \textbf{Method} & I-JEPA &  +\texttt{[CLS]}\\
    \midrule
    \textbf{ImageNet} & 72.4 & 72.4 \\
    \bottomrule
  \end{tabular}
\end{minipage}\hfill
\begin{minipage}[t]{0.58\linewidth}
  \centering
  \caption{\textbf{Effects of different attentions.}}
  \label{tab:atten_strategy}
    \begin{tabular}{ccc}
    \toprule
    \textbf{Method} & gradient-based &  \texttt{[CLS]}-based\\
    \midrule
    \textbf{ImageNet} & 73.4 & 73.5 \\
    \bottomrule
  \end{tabular}
\end{minipage}
\end{table}
